Towards Evaluating Adaptivity of Model-Based Reinforcement Learning Methods

In recent years, a growing number of deep model-based reinforcement learning (RL) methods have been introduced. The interest in deep model-based RL is not surprising, given its many potential benefits, such as higher sample efficiency and the potential for fast adaption to changes in the environment. However, we demonstrate, using an improved version of the recently introduced Local Change Adaptation (LoCA) setup, that well-known model-based methods such as PlaNet and DreamerV2 perform poorly in their ability to adapt to local environmental changes. Combined with prior work that made a similar observation about the other popular model-based method, MuZero, a trend appears to emerge, suggesting that current deep model-based methods have serious limitations. We dive deeper into the causes of this poor performance, by identifying elements that hurt adaptive behavior and linking these to underlying techniques frequently used in deep model-based RL. We empirically validate these insights in the case of linear function approximation by demonstrating that a modified version of linear Dyna achieves effective adaptation to local changes. Furthermore, we provide detailed insights into the challenges of building an adaptive nonlinear model-based method, by experimenting with a nonlinear version of Dyna.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\mathbf{0}}}
\def\vone{{\mathbf{1}}}
\def\vmu{{\bm{\mu}}}
\def\valpha{{\bm{\alpha}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\mathbf{a}}}
\def\vb{{\mathbf{b}}}
\def\vc{{\mathbf{c}}}
\def\vd{{\mathbf{d}}}
\def\ve{{\mathbf{e}}}
\def\vf{{\mathbf{f}}}
\def\vg{{\mathbf{g}}}
\def\vh{{\mathbf{h}}}
\def\vi{{\mathbf{i}}}
\def\vj{{\mathbf{j}}}
\def\vk{{\mathbf{k}}}
\def\vl{{\mathbf{l}}}
\def\vm{{\mathbf{m}}}
\def\vn{{\mathbf{n}}}
\def\vo{{\mathbf{o}}}
\def\vp{{\mathbf{p}}}
\def\vq{{\mathbf{q}}}
\def\vr{{\mathbf{r}}}
\def\vs{{\mathbf{s}}}
\def\vt{{\mathbf{t}}}
\def\vu{{\mathbf{u}}}
\def\vv{{\mathbf{v}}}
\def\vw{{\mathbf{w}}}
\def\vx{{\mathbf{x}}}
\def\vy{{\mathbf{y}}}
\def\vz{{\mathbf{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\mathbf{A}}}
\def\mB{{\mathbf{B}}}
\def\mC{{\mathbf{C}}}
\def\mD{{\mathbf{D}}}
\def\mE{{\mathbf{E}}}
\def\mF{{\mathbf{F}}}
\def\mG{{\mathbf{G}}}
\def\mH{{\mathbf{H}}}
\def\mI{{\mathbf{I}}}
\def\mJ{{\mathbf{J}}}
\def\mK{{\mathbf{K}}}
\def\mL{{\mathbf{L}}}
\def\mM{{\mathbf{M}}}
\def\mN{{\mathbf{N}}}
\def\mO{{\mathbf{O}}}
\def\mP{{\mathbf{P}}}
\def\mQ{{\mathbf{Q}}}
\def\mR{{\mathbf{R}}}
\def\mS{{\mathbf{S}}}
\def\mT{{\mathbf{T}}}
\def\mU{{\mathbf{U}}}
\def\mV{{\mathbf{V}}}
\def\mW{{\mathbf{W}}}
\def\mX{{\mathbf{X}}}
\def\mY{{\mathbf{Y}}}
\def\mZ{{\mathbf{Z}}}
\def\mBeta{{\mathbf{\beta}}}
\def\mPhi{{\mathbf{\Phi}}}
\def\mLambda{{\mathbf{\Lambda}}}
\def\mSigma{{\mathbf{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/LoCA_setups.tex <==
\section{LoCA setups}

A LoCA setup is a combination of three elements, an experimental setting, an environment, and a change of the environment. The experimental setting includes the number of time steps for training before and after the environment changes, some metric to evaluate the agent's performance, etc. The environment is a normal reinforcement learning environment, and the change of the environment is the change in the reward or the dynamics of the environment, with the state space and action space unchanged. We call a setup (with the above three elements) a LoCA setup if and only if:

\begin{itemize}
    \item The change of the environment changes good policies for the environment significantly.
    \item The change of the environment is local: only few small parts of environment are changed.
    \item After the environment changes, the agent observes only the changed parts of the environment, or small parts of the environment that cover the changes.
\end{itemize}

 This can be done, for example, by making the changed parts of the environment self-attractive.

We present multiple exemplary LoCA setups in this section. All the setups involve environments that require function approximation to solve.

\subsection{MountainCarLoCA}
The MountainCarLoCA setup involves a variant of the mountaincar environment. The state and action spaces, as well as the dynamics of the environment is the same as the original mountaincar environment, except that we 1) in addition to the terminal state at the top of the hill, add one more terminal state at the bottom of the hill with the velocity being close to 0, 2) reset the agent if a predefined timeout 500 is reached, and 3) to choose the initial state, uniformly sample from the state space for training and uniformly sample from a small region between the two terminal states and velocity close to 0 for evaluation. The agent receives a reward of 4 when the agent hits the terminal state at the top of the hill and receives a reward of 2 if it hits the terminal state at the bottom of the hill.

The only change of the environment is to change the reward when reaching the top of the hill from 4 to 0.

The experimental setting: 5 training runs, each run consists of 2e6 steps before the environment changes (phase 1) and 2e6 steps, the environment changes (phase 2), every 10000 steps we perform 5 evaluation runs and record the number of steps each run achieves the terminal state at the bottom of the hill (if this terminal state is not achieved, this number is equal to infty). We consider the average steps of reaching the correct terminal state over 10 evaluation runs. If the average is not too much worse than some predefined threshold, we treat these 10 evaluation runs successful. The threshold steps that we obtained are (50, 65, 80, 110) * 1.5 for stochasticity = 0.0, 0.1, 0.3, and 0.5 respectively. These numbers 50, 65, 80, 110 are obtained by running using sarsa($\lambda$) for a sufficient amount of time. The 1.5 scaling is a nice parameter to allow some sub-optimality. \textcolor{red}{How about recording the percentage of steps that the tested algorithms need more than sarsa($\lambda$)?}

\section{TODO}
\begin{enumerate}
    \item Find solver for the MC problem.
    \item Figure out why 10 tilings make the algorithm difficult to achieve 0 LoCA regret.
\end{enumerate}

==> tex/introduction.tex <==
\section{Introduction}
We provide an empirical study of several model-based algorithms with function approximation in several LoCA setups.

The LoCA paper (van Sejien et al.\ 2020) proposed LoCA setups to test if a reinforcement learning algorithm has the ability to adapt quickly when an environment changes, by \emph{only} observing the changed part of the environment. Such an ability can be achieved by planning with a learned model. It may also be achieved because the learned policy in the old environment also performs well in the new one. The first case is general and is independent of the environment or the change of the environment. The second case is a naive one. It happens only when the change of the environment does not change the policies that achieve high return in the environment. LoCA setup precludes this case by carefully designing the change of the environment so that the old policy is no longer a good one in the new environment. There may be a third case, in which an algorithm does not explicitly learn a model, but uses some mechanism that shares similar functionality as a model, and may still pass the test under the LoCA setup (e.g., predictive state representation, experience replay, etc). In fact, it may not be necessary to differentiate the first case and the third case, if one only cares about the \emph{behavior}, not the internal mechanism of an algorithm. LoCA test uses only the behavior of the agent. 

Building upon the original LoCA paper, one proposed contribution of this project is to introduce a clearer, simpler, and more general definition of LoCA setups, LoCA tests, LoCA regret etc. Formally speaking, we define a LoCA setup to be a combination of three elements: an experimental setting, an environment, and a change of the environment. A LoCA test is the evaluation of a complete algorithm (with all algorithmic hyper-parameters specified), in a LoCA setup, which produces either a single non-negative scalar, called \emph{LoCA regret}, or an \emph{unknown} flag. The unknown flag is generated if the algorithm does not perform sufficiently well even in the old environment. The LoCA regret is determined by the performance of the learned policy in the new environment, with 0 LoCA regret meaning that a sufficiently policy is obtained.
% We are interested in 1) designing several LoCA setups 2) finding algorithms that can achieve 0 LoCA regret under these LoCA setups, 3) analyzing algorithmic properties that are important in terms of achieving 0 LoCA regret.

Not all setups with the three components are LoCA setups. The change of the environment in the LoCA setup is designed to be \emph{local}, so that the change only happens in a small region of the possibly large environment state space and the agent can only observe real transitions from a small region of the environment when the change happens and has to largely rely on its model of the old environment to determine a good policy for the new environment.

An immediate follow-up question is what algorithms could possibly achieve 0 LoCA regret. A clearly understood case is the tabular Dyna algorithm, which is an algorithm that learns a model and plans with the learned model using value iteration. van Sejien\ et al. 2020 showed that this algorithm achieves 0 LoCA regret in a LoCA setup involving the Corridol domain. With function approximation (FA), however, some empirical results presented by van Sejien\ et al. 2020 showed that neither a state-of-the-art model-based algorithm, MuZero, or a simple classic model-free algorithm, Sarsa($\lambda$), can pass the test in a LoCA setup involving the MountainCar domain. The difficulties for a FA algorithm to adapt quickly in a LoCA setup are 1) the environments that require FA algorithms to deal with are typically more challenging 2) before the environment changes, the agent may keep only useful information for the old environment and ignore information that are useful for the new environment, due to the limited capacity of the FA.

The proposed contributions of this project are 1) clearly defining LoCA setups, LoCA tests, LoCA regret, etc, 2) design several LoCA setups that require FA algorithms 3) find FA algorithms that can achieve 0 LoCA regret in one or multiple of these LoCA setups, 4) analyze algorithmic properties are important in terms of achieving 0 LoCA regret.


==> tex/linear_dyna.tex <==

\section{Linear Dyna}
This algorithm is dyna with linear value function and linear models. We first provide the pseudo code of the algorithm. And later we show experimental results of the algorithm in the mountain-car LoCA setup. The results show that the algorithm achieves 0 LoCA regret with some hyper-parameters.

\begin{algorithm}[h]
\DontPrintSemicolon
\SetAlgoLined
\KwIn{exploration parameter $\epsilon$, stepsize $\alpha$, a feature mapping $\phi: \calS \to \bbR^m$ that produces from a state $s$ the corresponding $m$-sized feature vector $\phi(s)$, and a search control $d$.}
\SetKwInput{AP}{Algorithm parameters}
\SetKwRepeat{Do}{do}{while}
Initialize $\theta \in \bbR^m, F_a \in \bbR^m \times \bbR^m, b_a \in \bbR^m, \forall a \in \calA$ arbitrarily (e.g., to zero)\\
Obtain initial state $S$, Compute feature vector $\phi$ from $S$.\\
\While{still time to train}
{
    $A \gets \epsilon \text{-greedy} (b^\top_a \phi + \gamma F^\top_a \phi)$\\
    Take action $A$, receive reward $R$, next state $S'$, and termination $Z$. \\
    Compute the next feature vector $\phi'$ from $S'$.\\
    \If{$A$ is greedy} 
    {
        $\delta \gets r + \gamma (1 - Z) \theta^\top \phi' - \theta^\top \phi$\\
        $\theta \gets \theta + \alpha \delta \phi$\\
    }
    $F_A \gets F_A + \alpha ((1 - Z)\phi' - F_A \phi) \phi^\top$\\
    $b_A \gets b_A + \alpha (r - b_A^\top \phi) \phi$\\
    \For{all of the $n$ planning steps}
    {
        Generate a start feature vector $x$ by search control $d$\\
        $\delta \gets \max_a (b_a^\top x + \gamma  \theta^\top F_a^\top x) - \theta^\top x$\\
        $\theta \gets \theta + \alpha \delta x$\\
    }
    $\phi \gets \phi'$\\
}
% return $\theta, F_a, b_a, \forall a \in \calA$
\caption{Linear Dyna}
\label{algo:linear dyna}
\end{algorithm}

The exploration parameter $\epsilon \in [0.1, 0.5, 1.0]$, stepsize $\alpha \in [0.05, 0.1, 0.2]$. We used 3 different tile coding feature mappings, all of which produce similar length of feature vectors (approx. 1000). We used Tile Coding Software version 3.0beta by Sutton (http://www.incompleteideas.net/tiles/tiles3.html).

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c|c|c}
        Number of Tilings & 3 & 5 & 10 \\
        Tiling Size & 18 by 18 & 14 by 14 & 10 by 10
    \end{tabular}
    \caption{Tile Coding Setups}
    \label{tab: tile coding setups}
\end{table}

We tried 5 different ways to do search control
\begin{enumerate}
    \item \textbf{Random Feature Vector}: ask the environment to produce a random feature vector.
    \item \textbf{Experience Replay}: store \emph{all} the visited feature vectors in a buffer and uniformly sample from the buffer when we need a feature vector.
    \item \textbf{Grid Experience Replay}: map every state to a cell in a predefined grid. Whenever a state is visited, we put the state into the corresponding cell if the cell is empty. If the cell is not empty, we replace the state in the cell by the current state. To produce a feature vector, we randomly obtain a non-empty cell, and then generate the feature vector of the stored state.
    \item \textbf{Random Tabular Feature Vector}: produce a tabular (one-hot) feature vector with the 1-bit being randomly assigned.
    \item \textbf{Prioritize Sweeping}: see Algorithm 4 by Sutton et al.\ (2008) for details.
\end{enumerate}

We now present the experimental results for these different tilings.

\begin{figure}[h!]
\centering
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/random feature vector, a comparison of different tilings, epsilon 0.5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/random feature vector, a comparison of different epsilons, num_tilings 5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/random feature vector, a comparison of different stepsizes, num_tilings 5, epsilon 0.5.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/random feature vector.pdf}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{random feature vectors} with some hyper-parameters can achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2e6. 1) a comparison of different ways of tile coding with $\epsilon = 0.5, \alpha = 0.1$, 2) a comparison of different $\epsilon$s with 5 number of tilings and $\alpha = 0.1$, 3) a comparison of different stepsizes with 5 number of tilings and $\epsilon = 0.5$, 4) all curves.}
\label{fig: random feature vector}
\end{figure}

\begin{figure*}[h!]
\centering
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, a comparison of different tilings, epsilon 0.5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, a comparison of different epsilons, num_tilings 5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, a comparison of different stepsizes, num_tilings 5, epsilon 0.5.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay.pdf}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{experience replay} with some hyper-parameters can achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2e6. 1) a comparison of different ways of tile coding with $\epsilon = 0.5, \alpha = 0.1$, 2) a comparison of different $\epsilon$s with 5 number of tilings and $\alpha = 0.1$, 3) a comparison of different stepsizes with 5 number of tilings and $\epsilon = 0.5$, 4) all curves.}
\label{fig: experience replay}
\end{figure*}

\begin{figure*}[h!]
\centering
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, a comparison of different tilings, epsilon 0.5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, a comparison of different epsilons, num_tilings 5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, a comparison of different stepsizes, num_tilings 5, epsilon 0.5.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay.pdf}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{grid experience replay} with some hyper-parameters can achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2e6. 1) a comparison of different ways of tile coding with $\epsilon = 0.5, \alpha = 0.1$, 2) a comparison of different $\epsilon$s with 5 number of tilings and $\alpha = 0.1$, 3) a comparison of different stepsizes with 5 number of tilings and $\epsilon = 0.5$, 4) all curves.}
\label{fig: grid experience replay}
\end{figure*}


\begin{figure*}[h!]
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/tabular feature, a comparison of different tilings, epsilon 0.5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/tabular feature, a comparison of different epsilons, num_tilings 5, alpha 0.1.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/tabular feature, a comparison of different stepsizes, num_tilings 5, epsilon 0.5.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/tabular feature.pdf}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{tabular feature vectors} do not achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2e6. 1) a comparison of different ways of tile coding with $\epsilon = 0.5, \alpha = 0.1$, 2) a comparison of different $\epsilon$s with 5 number of tilings and $\alpha = 0.1$, 3) a comparison of different stepsizes with 5 number of tilings and $\epsilon = 0.5$, 4) all curves.}
\label{fig: tabular feature}
\end{figure*}


\begin{figure}[h!]
\centering
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/prioritize sweeping, a comparison of different tilings, epsilon 0.5, alpha 0.1.pdf}
    \caption{Comparison of different tilings}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/prioritize sweeping, a comparison of different epsilons, num_tilings 5, alpha 0.1.pdf}
    \caption{Comparison of different epsilons}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/prioritize sweeping, a comparison of different stepsizes, num_tilings 5, epsilon 0.5.pdf}
    \caption{Comparison of different stepsizes}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/prioritize sweeping.pdf}
    \caption{All}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{prioritize sweeping} do not achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2e6. 1) a comparison of different ways of tile coding with $\epsilon = 0.5, \alpha = 0.1$, 2) a comparison of different $\epsilon$s with 5 number of tilings and $\alpha = 0.1$, 3) a comparison of different stepsizes with 5 number of tilings and $\epsilon = 0.5$, 4) all curves.}
\label{fig: tabular feature}
\end{figure}

\subsection{Finer Tilings}

We further tested the algorithm with finer tile coding, with 10 number of tilings, with each tiling being a 20 by 20 grid. However, this finer tile coding still can not achieve 0 LoCA regret.

\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay with 10 20 by 20 tilings.pdf}
    \caption{Grid experience replay}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/random feature vector with 10 20 by 20 tilings.pdf}
    \caption{Random feature vector}
\end{subfigure}
\caption{Plots showing learning curves using grid experience replay or random feature vector with \textbf{10 20 by 20 tilings} do not achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 1.2 * 1e5. 1) all curves with grid experience replay 2) all curves with random feature vector}
\label{fig: finer tilings}
\end{figure}

\subsection{Stochasticity}

We now present a new set of experiments testing the algorithm in the stochastic mountain car domain, with 5 number of tilings, with each tiling being a 10 by 10 grid. We tried a larger timeout 1000 to make sure that the agent achieves the goal within timeout.

\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.0, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.0, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.1, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0.1}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.1, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0.1}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.3, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0.3}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.3, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0.3}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.5, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0.5}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/grid experience replay, stochasticity 0.5, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0.5}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{grid experience replay} with 5 10 by 10 tilings can achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 20000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2 * 1e6. The left columns are those with timeout 500 and the right columns are those with timeout 1000. Each row corresponds to one choice of stochasticity (0, 0.1, 0.3, 0.5).}
\label{fig: grid experience replay stochasticity}
\end{figure}

\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.0, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.0, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.1, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0.1}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.1, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0.1}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.3, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0.3}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.3, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0.3}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.5, timeout 500.pdf}
    \caption{Timeout: 500, Stochasticity: 0.5}
\end{subfigure}
\begin{subfigure}[t]{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, stochasticity 0.5, timeout 1000.pdf}
    \caption{Timeout: 1000, Stochasticity: 0.5}
\end{subfigure}
\\
\caption{Plots showing learning curves using \textbf{experience replay} with 5 10 by 10 tilings can achieve 0 LoCA regret. The $x$ axis is the number of training steps. Every 20000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 5 runs, and plot the rate of moving to terminal 2. The second phase starts from 2 * 1e6. The left columns are those with timeout 500 and the right columns are those with timeout 1000. Each row corresponds to one choice of stochasticity (0, 0.1, 0.3, 0.5).}
\label{fig: experience replay stochasticity}
\end{figure}

\section{TODO}
\subsection{Report}
\subsubsection{Effect of Stepsizes}
\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing stepsizes, stochasticity = 0.0, timeout 500, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing stepsizes, stochasticity = 0.1, timeout 500, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing stepsizes, stochasticity = 0.3, timeout 500, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.3}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing stepsizes, stochasticity = 0.5, timeout 500, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.5}
\end{subfigure}
\caption{Plots showing learning curves using a \textbf{relatively smaller stepsize} achieves better adaptation in the second phase. There are 5 14 by 14 tilings. $\epsilon = 0.5$, Timeout = 500. The actual stepsizes are re-scaled by the number of tilings (5). The The $x$ axis is the number of training steps. For each experiment, we performed 5 independent runs. Each run lasts for 4 * 1e6 training steps. Every 20000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 10 testing runs, and plot the average steps the agent uses to move to terminal 2 (if it moves to terminal 1, then the number of steps is 1000). The second phase starts from 2 * 1e6. We also plot the average steps used by sarsa($\lambda$), after training for sufficiently long (optimal policy).}
\label{fig: experience replay stochasticity}
\end{figure}

\subsubsection{Effect of Epsilon}
\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing epsilons, stochasticity = 0.0, stepsize = 0.1, timeout 500, number of tilings = 5.pdf}
    \caption{Stochasticity = 0}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing epsilons, stochasticity = 0.1, stepsize = 0.1, timeout 500, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing epsilons, stochasticity = 0.3, stepsize = 0.1, timeout 500, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.3}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing epsilons, stochasticity = 0.5, stepsize = 0.1, timeout 500, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.5}
\end{subfigure}
\caption{Plots showing learning curves using \textbf{different $\epsilon$s}. There are 5 14 by 14 tilings. $\epsilon = 0.5$, $\alpha = 0.1$. The actual stepsizes are re-scaled by the number of tilings (5). The The $x$ axis is the number of training steps. For each experiment, we performed 5 independent runs. Each run lasts for 4 * 1e6 training steps. Every 20000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 10 testing runs, and plot the average steps the agent uses to move to terminal 2 (if it moves to terminal 1, then the number of steps is 1000). The second phase starts from 2 * 1e6. We also plot the average steps used by sarsa($\lambda$), after training for sufficiently long (optimal policy). The result is inconclusive because when stochasticity = 0.3, $\epsilon = 0.5$ is better while in all other three cases. $\epsilon = 1$ is better. I think this is because only 5 runs are done and $\epsilon = 0.5$ is lucky when stochasticity = 0.3.}
\label{fig: experience replay stochasticity}
\end{figure}

\subsubsection{Effect of Timeout}

\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing timeouts, stochasticity = 0.0, stepsize = 0.1, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing timeouts, stochasticity = 0.1, stepsize = 0.1, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing timeouts, stochasticity = 0.3, stepsize = 0.1, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.3}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay, comparing timeouts, stochasticity = 0.5, stepsize = 0.1, epsilon = 0.5, number of tilings = 5.pdf}
    \caption{Stochasticity = 0.5}
\end{subfigure}
\caption{Plots showing learning curves using a \textbf{larger timeout} achieves more stable adaptation in the second phase. There are 5 14 by 14 tilings. $\epsilon = 0.5$, $\alpha = 0.1$. The actual stepsizes are re-scaled by the number of tilings (5). The The $x$ axis is the number of training steps. For each experiment, we performed 5 independent runs. Each run lasts for 4 * 1e6 training steps. Every 20000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 10 testing runs, and plot the average steps the agent uses to move to terminal 2 (if it moves to terminal 1, then the number of steps is 1000). The second phase starts from 2 * 1e6. We also plot the average steps used by sarsa($\lambda$), after training for sufficiently long (optimal policy).}
\label{fig: experience replay stochasticity}
\end{figure}

\subsubsection{Effect of Number of Tilings}
Waiting for results.

\subsection{Return curves}
Waiting for results.

\subsection{Analyzing Number of Tiling = 10}
Computing model error averaged over the entire state space to see if the average error diverge in phase 2. Use a separate model learning rate. Waiting for results.

\section{New Results}
\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay best.pdf}
    \caption{Best}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay buffer size.pdf}
    \caption{Buffer Size}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay epsilon.pdf}
    \caption{$\epsilon$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay tiling.pdf}
    \caption{Tiling}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay lr.pdf}
    \caption{$\alpha$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay model lr.pdf}
    \caption{$\beta$}
\end{subfigure}
\caption{Plots showing learning curves in the deterministic mountaincar environment. The The $x$ axis is the number of training steps. For each experiment, we performed 10 independent runs. Each run lasts for 4e6 training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 10 testing runs, and plot the discounted return. The second phase starts from 2e6. We also plot the best return achieved by sarsa($\lambda$), after training for sufficiently long (optimal policy).}
\label{fig: experience replay stochasticity}
\end{figure}

\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay best stoch 0.3.pdf}
    \caption{Best}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay buffer size stoch 0.3.pdf}
    \caption{Buffer Size}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay epsilon stoch 0.3.pdf}
    \caption{$\epsilon$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay tiling stoch 0.3.pdf}
    \caption{Tiling}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay lr stoch 0.3.pdf}
    \caption{$\alpha$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay model lr stoch 0.3.pdf}
    \caption{$\beta$}
\end{subfigure}
\caption{Plots showing learning curves in the stochastic mountaincar environment (0.3). The The $x$ axis is the number of training steps. For each experiment, we performed 10 independent runs. Each run lasts for 4e6 training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 10 testing runs, and plot the discounted return. The second phase starts from 2e6. We also plot the best return achieved by sarsa($\lambda$), after training for sufficiently long (optimal policy).}
\label{fig: experience replay stochasticity}
\end{figure}

\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay best stoch 0.5.pdf}
    \caption{Best}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay buffer size stoch 0.5.pdf}
    \caption{Buffer Size}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay epsilon stoch 0.5.pdf}
    \caption{$\epsilon$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay tiling stoch 0.5.pdf}
    \caption{Tiling}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay lr stoch 0.5.pdf}
    \caption{$\alpha$}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/experience replay model lr stoch 0.5.pdf}
    \caption{$\beta$}
\end{subfigure}
\caption{Plots showing learning curves in the stochastic mountaincar environment (0.3). The The $x$ axis is the number of training steps. For each experiment, we performed 10 independent runs. Each run lasts for 4e6 training steps. Every 10000 training steps, we evaluate the agent's greedy policy with the initial state distribution being \emph{init eval} for 10 testing runs, and plot the discounted return. The second phase starts from 2e6. We also plot the best return achieved by sarsa($\lambda$), after training for sufficiently long (optimal policy).}
\label{fig: experience replay stochasticity}
\end{figure}
